Optimal sports betting strategies in practice: an experimental review

We investigate the most popular approaches to the problem of sports betting investment based on modern portfolio theory and the Kelly criterion. We define the problem setting, the formal investment strategies, and review their common modifications used in practice. The underlying purpose of the reviewed modifications is to mitigate the additional risk stemming from the unrealistic mathematical assumptions of the formal strategies. We test the resulting methods using a unified evaluation protocol for three sports: horse racing, basketball and soccer. The results show the practical necessity of the additional risk-control methods and demonstrate their individual benefits. Particularly, we show that an adaptive variant of the popular ``fractional Kelly'' method is a very suitable choice across a wide range of settings.

==> acknowledgment.tex <==
Acknowledgements
The authors acknowledge support by grant no. 20-29260S from the Czech Science Foundation

==> backup/refs.tex <==
\begin{thebibliography}{10}

\bibitem[Axelsson(1994)Axelsson]
{BAxe94}
\textsc{Axelsson, O.} (1994)
\newblock \emph{Iterative Solution Methods}.
\newblock Cambridge: Cambridge University Press.

\bibitem[Axelsson \& Lindskog(1986a)Axelsson \& Lindskog]
{Axe86}
\textsc{Axelsson, O. \& Lindskog, G.} (1986a)
\newblock On the eigenvalue distribution of a class of preconditioning
methods.
\newblock \emph{Numer. Math.}, \textbf{48}, 479--498.

\bibitem[Axelsson \& Lindskog(1986b)Axelsson \& Lindskog]
{Axe86b}
\textsc{Axelsson, O. \& Lindskog, G.} (1986b)
\newblock On the rate of convergence of the preconditioned conjugate
gradient method.
\newblock \emph{Numer. Math.}, \textbf{48}, 499--523.

\bibitem[Bebendorf \& Hackbusch(2003)Bebendorf \& Hackbusch]
{Bebendorf03}
\textsc{Bebendorf, M. \& Hackbusch, W.} (2003)
\newblock Existence of $H$-matrix approximants to the inverse FE matrix
of elliptic operators with $L^\infty$-coefficients.
\newblock \emph{Numer. Math.}, \textbf{95}, 1--28.

\bibitem[Beckermann \& Kuijlaars(2001)Beckermann \& Kuijlaars]
{Beckermann01}
\textsc{Beckermann, B. \& Kuijlaars, A. B. J.} (2001)
\newblock Superlinear convergence of conjugate gradients.
\newblock \emph{SIAM J. Numer. Anal.}, \textbf{39}, 300--329.

\bibitem[Beckermann \& Kuijlaars(2002)Beckermann \& Kuijlaars]
{Beckermann02}
\textsc{Beckermann, B. \& Kuijlaars, A. B. J.} (2002)
\newblock Superlinear CG convergence for special right-hand sides.
\newblock \emph{Electron. Trans. Numer. Anal.}, \textbf{14}, 1--19.
\newblock Special volume on orthogonal polynomials, approximation theory,
and harmonic analysis (Inzell, 2000).

\bibitem[Bramble \emph{et al.}(1991)Bramble, Pasciak, Wang \& Xu]
{Bra91}
\textsc{Bramble, J. H., Pasciak, J. E., Wang, J. \& Xu, J.} (1991)
\newblock Convergence estimates for multigrid algorithms without regularity
assumptions.
\newblock \emph{Math. Comp.}, \textbf{57}, 23--45.

\bibitem[Cai \emph{et al.}(1999)Cai, Nielsen \& Tveito]
{Cai99}
\textsc{Cai, X., Nielsen, B. F. \& Tveito, A.} (1999)
\newblock An analysis of a preconditioner for the discretized pressure
equation arising in reservoir simulation.
\newblock \emph{IMA J. Numer. Anal.}, \textbf{19}, 291--316.

\bibitem[Chan \& Mathew(1994)Chan \& Mathew]
{Cha94}
\textsc{Chan, T. F. \& Mathew, T. P.} (1994)
\newblock Domain decomposition algorithms.
\newblock \emph{Acta Numer.}, 61--143.

\bibitem[Dryja(1994)Dryja]
{Dry94b}
\textsc{Dryja, M.} (1994)
\newblock Multilevel methods for elliptic problems with discontinuous
coefficients in three dimensions.
\newblock \emph{Domain Decomposition Methods in Scientific and Engineering Computing}
(D. E. Keyes \& J. Xu eds).
\newblock Providence, RI: American Mathematical Society,
pp.\ 43--47.

\bibitem[Dryja \emph{et al.}(1996)Dryja, Sarkis \& Widlund]
{Dry94}
\textsc{Dryja, M., Sarkis, M. \& Widlund, O. B.} (1996)
\newblock Multilevel Schwarz methods for elliptic problems with
discontinuous coefficients in three dimensions.
\newblock \emph{Numer. Math.}, \textbf{72}, 313--348.

\bibitem[Graham \& Hagger(1999)Graham \& Hagger]
{Gra99}
\textsc{Graham, I. G. \& Hagger, M. J.} (1999)
\newblock Unstructured additive Schwarz-conjugate gradient method
for elliptic problems with highly discontinuous coefficients.
\newblock \emph{SIAM J. Sci. Comput.}, \textbf{20}, 2041--2066.

\bibitem[Griffel(1981)Griffel]
{BGri81}
\textsc{Griffel, D. H.} (1981)
\newblock \emph{Applied Functional Analysis}.
\newblock Chichester: Horwood.

\bibitem[Hackbusch(1994)Hackbusch]
{BHac94}
\textsc{Hackbusch, W.} (1994)
\newblock \emph{Iterative Solution of Large Sparse Systems of Equations}.
\newblock New York: Springer.

\bibitem[Langtangen(1999)Langtangen]
{BLan99}
\textsc{Langtangen, H. P.} (1999)
\newblock \emph{Computational Partial Differential Equations.
Numerical Methods and Diffpack Programming}.
\newblock Berlin: Springer.

\bibitem[Marti(1986)Marti]
{BMar86}
\textsc{Marti, J. T.} (1986)
\newblock \emph{Introduction to Sobolev Spaces and Finite Element
Solution of Elliptic Boundary Value Problems}.
\newblock London: Academic Press.

\bibitem[Naiman \emph{et al.}(1997)Naiman, Babu\v{s}ka \& Elman]
{Naiman97}
\textsc{Naiman, A. E., Babu\v{s}ka, I. M. \& Elman, H. C.} (1997)
\newblock A note on conjugate gradient convergence.
\newblock \emph{Numer. Math.}, \textbf{76}, 209--230.

\bibitem[Naiman \& Engelberg(2000)Naiman \& Engelberg]
{Naiman00}
\textsc{Naiman, A. E. \& Engelberg, S.} (2000)
\newblock A note on conjugate gradient convergence. II, III.
\newblock \emph{Numer. Math.}, \textbf{85}, 665--683, 685--696.

\bibitem[Royden(1989)Royden]
{BRoy89}
\textsc{Royden, H. L.} (1989)
\newblock \emph{Real Analysis}.
\newblock New York: Macmillan.

\bibitem[Stoer \& Bulirsch(1993)Stoer \& Bulirsch]
{BStoe93}
\textsc{Stoer, J. \& Bulirsch, R.} (1993)
\newblock \emph{Introduction to Numerical Analysis}.
\newblock New York: Springer.

\end{thebibliography}


==> backup/triangle.tex <==
\begin{tikzpicture}
\node[color=black, align=center] (Pr) [] {$P_r$ \\ $[p_{r_1}, \dots, p_{r_n}]$};
\node[color=black, align=center] (Pb) [below left= 1cm and 1cm of Pr] {$P_b$ \\ $[p_{b_1}, \dots, p_{b_n}]$};
\node[color=black, align=center] (Pp) [below right= 1cm and 1cm of Pr] {$P_p$ \\ $[p_{p_1}, \dots, p_{p_n}]$};

\draw [thick,<->] (Pr) edge node[above,sloped] { $D|P_r,P_b|$} (Pb);
\draw [thick,<->] (Pr) edge node[above,sloped] { $D|P_r,P_p|$} (Pp);
\draw [thick,<->] (Pb) edge node[below,sloped] { $D|P_b,P_p|$} (Pp);
\end{tikzpicture}


